A Flexible Framework for Defining, Representing and Detecting Changes on the Data Web

The dynamic nature of Web data gives rise to a multitude of problems related to the identification, computation and management of the evolving versions and the related changes. In this paper, we consider the problem of change recognition in RDF datasets, i.e., the problem of identifying, and when possible give semantics to, the changes that led from one version of an RDF dataset to another. Despite our RDF focus, our approach is sufficiently general to engulf different data models that can be encoded in RDF, such as relational or multi-dimensional. In fact, we propose a flexible, extendible and data-model-independent methodology of defining changes that can capture the peculiarities and needs of different data models and applications, while being formally robust due to the satisfaction of the properties of completeness and unambiguity. Further, we propose an ontology of changes for storing the detected changes that allows automated processing and analysis of changes, cross-snapshot queries (spanning across different versions), as well as queries involving both changes and data. To detect changes and populate said ontology, we propose a customizable detection algorithm, which is applicable to different data models and applications requiring the detection of custom, user-defined changes. Finally, we provide a proof-of-concept application and evaluation of our framework for different data models.

==> intro_prev.tex <==
\section{Introduction}
\label{sec:intro}

With the growing complexity of the WWW, we face a completely different way for creating, disseminating and consuming big volumes of information. Large-scale corporate, government, or even user-generated data are published and become available to a wide spectrum of users. DBpedia, Freebase, YAGO and Atlas are, among many others, examples of large data repositories, which store information about various entities, including their relationships. Typically, data in such datasets are represented using the RDF model~\cite{rdf}, in which information is stored in triples of the form (\textit{subject}, \textit{predicate}, \textit{object}), meaning that \textit{subject} is related to \textit{object} via \textit{predicate}. 
%For example, the Billion Triples Challenge dataset of 2012 contains about 1.44B triples, DBPedia v3.9, Freebase and Yago alone feature 25M, 40M and 10M entities, and 2.46B, 1.9B and 120M triples, respectively, while Atlas v13.07 contains about 447M triples \cite{ksteftut14}.

Dynamicity is an indispensable part of the current web; datasets are constantly evolving for several reasons, such as the inclusion of new experimental evidence or observations, or the correction of erroneous conceptualizations~\cite{freqevolution}. As an example, consider the detected number of changes between the versions 12.07 and 13.05, and 13.05 and 13.07 of Atlas which are 879.5M and 801.2M, respectively, while between the versions 3.7 and 3.8, and 3.8 and 3.9 of the English DBpedia are 20.7M and 9.3M (Figure~\ref{fig:results_changes}). 

This constant evolution poses several research problems, which are related to the identification, computation, storage and management of the evolving versions. 
An important question is how to support complex changes, whose constituent changes are seemingly unrelated and may occur on disparate pieces of data, but together as a whole they have a semantically coherent meaning for an application domain. 
Clearly, understanding and detecting the changes of evolving datasets is a prerequisite to address these problems. In particular, finding the differences (deltas) between datasets has been proved to play a crucial role in various curation tasks, such as the synchronization of autonomously developed datasets versions~\cite{DBLP:Cloran2005}, or the visualization of the evolution history of a dataset~\cite{DBLP:Noy2006}. 
Deltas are also necessary in certain applications that require access to previous versions of a dataset to support historical or cross-snapshot queries (e.g.,~\cite{DBLP:conf/er/StefanidisCF14}), in order, for example, to identify past states of the dataset, understand the evolution process, or detect the source of errors in the current modelling.

In general, there are two ways to record the occurring changes. The first is by constantly \textit{monitoring} the dataset and logging any change, which requires a closed and controlled system, where all changes pass through a dedicated application that records every change as it happens. 
A more flexible method includes \textit{detecting} a posteriori the changes that happened. This avoids the need to have a controlled system, and allows remote users of a dataset to identify changes, even if they have no access to the actual change process or knowledge that it happened. 
Here, we focus on the latter case, which is more challenging and interesting, even though most of the proposed solutions (namely, the definition of a language of changes and the representation of the changes) are applicable in both scenarios.

Detection of changes is based on 3 main pillars, namely \textit{defining}, \textit{representing} and \textit{detecting} changes. 
The first pillar (defining changes) is related to the definition of a \textit{language of changes}, which is based on the set of changes that are understandable by the system. Defining the language of changes includes identifying the types of changes that will be detected, their formal definition (e.g., their semantics and parameters), and takes into account the need for complex, domain-specific changes. It has been argued that the language of changes as a whole, should be well-behaved in the sense of satisfying certain properties, namely being \textit{complete and unambiguous}, so as to allow the generation of unique deltas in a deterministic manner~\cite{DBLP:journals/tods/PapavasileiouFFKC13}.
The definition of changes is given in Section~\ref{sec:define}.

The second pillar (representing changes) is related to the representation scheme used for storing the detected changes. This is necessary to allow a persistent representation and storage of the detected changes, as well as to support navigation among versions, analysis of the deltas, cross-snapshot or historic queries, and the raising of changes as first class citizens in a multi-version repository. Our approach is based on the definition of an \textit{ontology of changes} that satisfies these goals.
The representation scheme of the proposed changes is given in Section~\ref{sec:represent}.

Finally, the third pillar (detecting changes) is related to the algorithmic definition of the detection process. This process identifies the changes applied between any two versions, based on the actual change definitions in the language of changes, and stores the results in the ontology of changes. Our approach for change detection is based on the execution of appropriately defined SPARQL queries, whose answers determine the detected changes.
Details on the detection process are given in Section~\ref{sec:detect}.

One of the major challenges related to change detection and deltas is that no language of changes is suitable for all different applications and models.
There are two reasons for that. First, the different types of data available on the Web are often represented using different data models, which call for different changes.
Second, different uses (or users) of the data may require a different set of changes being reported, or the definition of special types of changes that happen often or are important for the operation of the data-driven application. 
Therefore, there is no one-size-fits-all solution for the problem of change detection.

In this work, we propose a flexible framework for change detection that can be applied to different models and applications. Our intention is not to provide a single solution, but a generic methodology for defining the three components of a multi-version repository, through which different solutions, suitable for different needs, can be developed. 
Even though our framework is designed for RDF, our approach is applicable to any data model representable in RDF, i.e., RDF is used as a unifying underlying model to achieve this generality.

Regarding the definition of changes, the objective of generality is met by providing two different types of changes, namely \textit{simple} and \textit{complex} (see Section~\ref{sec:define}). The former type is meant to capture fine-grained changes for the data model at hand, and should meet the requirements of completeness and unambiguity; towards this aim, we provide a generic methodology for determining whether a proposed set of simple changes has these properties.
The latter type is meant to capture more coarse-grained changes, or specialized changes that are useful for the application at hand; this allows a customized behaviour of the change detection process, depending on the actual needs of the application. Complex changes are totally dynamic, and can be defined even at run-time, greatly enhancing the flexibility of our approach. 

For the purposes of representation, the proposed ontology of changes is designed to be generic enough, so as to be customizable for different languages of changes.
This allows us to meet the aforementioned generality goal, as detailed in Section~\ref{sec:represent}. 
The detection process is defined in a customizable manner, as the core detection algorithm is agnostic to the actual set of simple or complex changes used. The customization for the actual language of changes employed is based on the definition of appropriate SPARQL queries (one per change) that come as parameters to the algorithm, thereby allowing new changes to be easily defined. Details are given in Section~\ref{sec:detect}.

An additional contribution is the application of this work for data models other than the pure RDF model, namely the multi-dimensional model that have been transformed to the RDF Data Cube vocabulary, while it could be also applied similarly to the relational model. This application is meant as a proof-of-concept that the proposed approach is indeed capable of supporting diverse needs, and is not exhaustive in terms of the types of applications or models that our framework supports.

Finally, we provide experiments for these use cases showing that the most crucial parameter in the change detection process is the total number of detected changes rather than the size of the examined datasets. Also, we prove that the number of simple changes is proportional to the number of triples which will be inserted into the ontology. Except from the evaluation aspect of our framework, our experiments provide a detailed look on the evolution of real-world, big datasets, as we record changes and provide an analysis of their form. The proposed approach extends our previous work on change detection~\cite{DBLP:journals/tods/PapavasileiouFFKC13}, by providing a more generic change definition framework; here, we experience significantly improved performance (about 1 order of magnitude), scalability, as well as increased generality and applicability.



%Finally, we provide experiments for these use cases showing that the most crucial parameter in the change detection process is the total number of detected changes rather than the size of the examined datasets. Also it proved that the number of simple changes is proportional to the number of triples which will be inserted into the ontology. Our work overcomes our previous one presented and evaluated in \cite{DBLP:journals/tods/PapavasileiouFFKC13} and it seems to be scalable and independent of any dataset.

%Except from the evaluation aspect of our framework, our experiments provide a detailed look on evolution of real world datasets, as we record changes and provide an analysis of their appearance.

%This paper can be seen as an extension and generalization of the previous work~\cite{DBLP:journals/tods/PapavasileiouFFKC13}. Compared to this work, we experience significantly improved performance \GF{be more specific here}, as well as increased generality and applicability. 


==> represent.tex <==
\section{Representing Changes}
\label{sec:represent}

Explain the ontology of changes, its features, and its advantages.

Give  it a name.

How linked data principles are used here to support cross-snapshot and similar queries (we have no experiments for that, so don't describe this as a contribution).

Put figures for the ontology of  changes. 

\YX{Apla shmeiwnw edw thn idea ths arxitektonikhs prin apo ta peiramata se periptwsh pou exoume xwro...}


